Running Alchemist on Cray XC and CS Series Supercomputers: Dask and PySpark Interfaces, Deployment Options, and Data Transfer Times

Alchemist is a system that allows Apache Spark to achieve better performance by interfacing with HPC libraries for large-scale distributed computations. In this paper, we highlight some recent developments in Alchemist that are of interest to Cray users and the scientific community in general. We discuss our experience porting Alchemist to container images and deploying it on Cray XC (using Shifter) and CS (using Singularity) series supercomputers and on a local Kubernetes cluster. Newly developed interfaces for Python, Dask, and PySpark enable the use of Alchemist with additional data analysis frameworks. We also briefly discuss the combination of Alchemist with RLlib, an increasingly popular library for reinforcement learning, and consider the benefits of leveraging HPC simulations in reinforcement learning. Finally, since data transfer between the client applications and Alchemist are the main overhead Alchemist encounters, we give a qualitative assessment of these transfer times with respect to different~factors.

==> Section_0_Long_Abstract.tex <==
% \section{Introduction}
\noindent Alchemist~\cite{Gittens2018b, Gittens2018a, alchemist2019} allows Apache Spark~\cite{Zaharia2016} to achieve better performance by interfacing with HPC libraries for large-scale distributed computations. In this paper we discuss some recent and current developments in Alchemist that are of interest to Cray users and the scientific community in general. 

\section{Deploying Alchemist on Different Platforms using Containers}

A container image allows us to bundle applications and their dependencies together into a single entity. This container image is deployed on a host machine to run the machine learning or analytics framework with Alchemist. Moving to a container-based deployment means users need not worry about building the applications from source and managing dependencies every time they want to run their application on a new platform. 

Docker~\cite{docker2018} is an open source container technology that has gained wide adoption. We discuss our experience porting Alchemist to a Dockerfile and then deploying it on Cray XC and CS series supercomputers, on a local cluster, and on the cloud.
\begin{itemize}
\item Cray XC series supercomputers use Shifter~\cite{shifter2018}, developed at NERSC to deploy container images. We show how we can adapt the Dockerfile so that we can deploy Alchemist on Cray XC and leverage the Cray MPI library stack.
\item Cray CS series supercomputers use Singularity~\cite{singularity2018} for launching container images on the nodes. Singularity provides the flexibility to import Docker images without having Docker installed or being a superuser. We leverage this ability to run Alchemist on CS systems with optimized OpenMPI libraries. 
\item Kubernetes~\cite{kubernetes2018} is an open source orchestration framework that supports running, scaling and management of containers and has gained popularity both on the cloud and on on-premises clusters. We demonstrate how the Alchemist Docker image is used with Kubernetes and run on a local Kubernetes cluster, as well as on a Kubernetes cluster deployed on a cloud provider like AWS. 
\end{itemize}
There are subtle differences between each of these flavors of container orchestration and this discussion will provide guidance for users on how to use their favorite container technology with Alchemist, as opposed to being restricted to one single mode of deployment.

\section{Python, DASK, and PySpark Interfaces}

Alchemist was originally written as an interface between Apache Spark and MPI-based libraries, but recent modifications have allowed client interfaces for other data analysis and machine learning frameworks to be easily developed. To this end, a Python interface has been written and serves as a basis for client interfaces currently being developed for DASK~\cite{dask}, a popular library that supports parallel computing in Python, and PySpark~\cite{pyspark2018}.

The ability to use Alchemist from these additional frameworks enables more users to easily connect to HPC libraries. We will describe the details of each of these interfaces and discuss the specific features that offer greater ease of use.

\section{RLlib + Alchemist for Reinforcement Learning with HPC Simulations}

Reinforcement learning (RL) is an increasingly popular machine learning technique that allows an agent to be trained by interacting with an environment and collecting rewards, with the goal being to maximize the number of accumulated rewards by the end of the training. The agent must find which actions to take to obtain the maximum number of rewards independently, and therefore, due to its trial-and-error approach, a large number of simulations are required in order to successfully train the agent. While the computational cost of these simulations may be unimportant when applying RL to small problems that are commonly used to illustrate its power, it becomes the major bottleneck when applying RL to large-scale problems in science and engineering that require significant computational resources.

RLlib~\cite{RLlib} is an open-source library that provides a collection of RL algorithms and scalable primitives for composing new ones. It has seen a significant increase in interest recently and we hope to combine RLlib with Alchemist to help facilitate the adoption of RL by the scientific and engineering communities. Alchemist would allow users to employ efficient HPC libraries for the simulations while still working with the extensive toolset and convenient interface provided by RLlib. 

\section{Evaluating Data Transmission Times}

As discussed in \cite{Gittens2018b}, the main computational overhead of Alchemist is the time it takes to transfer the data between the Spark application and the MPI-based libraries. A simple experiment to quantify these communication times for two 400GB matrices with different sizes was performed, see Tables 2 and 3 in~\cite{Gittens2018b}.

We want to perform a more comprehensive evaluation of these data transmission times with respect to the following criteria:
\begin{itemize}
    \item \textit{Matrix layout}: The experiments in the cited tables are for sending rows from an \texttt{IndexedRowMatrix} in Spark to a distributed Elemental~\cite{elemental2017} matrix having a column-major ordering of the 2D process grid (i.e. we are sending data from rows to rows). The layout used by the distributed matrices can have a significant impact on the performance of the MPI-based libraries, so it may be desirable to send the data from Spark to a distributed matrix that has a more favorable layout for the computations that are going to be performed on it. See~\cite{elemental2017doc} for a discussion of different matrix layouts that are possible with respect to the process grid. The layout that is used determines the size and number of messages sent between the client and Alchemist, which will impact the overall communication time. 
    \item \textit{Matrix dimension}: Both the size and aspect ratio (the height-to-width ratio of the matrix) affect the data transmission times. It was found in~\cite{Gittens2018b} that sending rows is more efficient if the matrix is short and wide. This is in part due to how the data was transferred by Alchemist at the time (which has now been improved to take this into account), but a more thorough investigation of what effect the matrix dimensions have will nonetheless be beneficial.
    \item \textit{Transmission time variability}: While performing the previous experiments, it was found that there is significant variability in the transmission times (the reported times were averages). This is due to the number of messages being sent between the client and Alchemist, with a larger number of shorter messages leading to transmission times that are significantly more variable, as one would expect. We will run experiments to better quantify this variability.
\end{itemize}

